Accurate Modeling of Lyman-alpha Profiles and their Impact on Photolysis of Terrestrial Planet Atmospheres

Accurately measuring and modeling the Lyman-$\alpha$ (Ly$\alpha$; $\lambda$1215.67 \AA) emission line from low mass stars is vital for our ability to build predictive high energy stellar spectra, yet interstellar medium (ISM) absorption of this line typically prevents model-measurement comparisons. Ly$\alpha$ also controls the photodissociation of important molecules, like water and methane, in exoplanet atmospheres such that any photochemical models assessing potential biosignatures or atmospheric abundances require accurate Ly$\alpha$ host star flux estimates. Recent observations of three early M and K stars (K3, M0, M1) with exceptionally high radial velocities (>100 km s$^{-1}$) reveal the intrinsic profiles of these types of stars as most of their Ly$\alpha$ flux is shifted away from the geocoronal line core and contamination from the ISM. These observations indicate that previous stellar spectra computed with the PHOENIX atmosphere code have underpredicted the core of Ly$\alpha$ in these types of stars. With these observations, we have been able to better understand the microphysics in the upper atmosphere and improve the predictive capabilities of the PHOENIX atmosphere code. Since these wavelengths drive the photolysis of key molecular species, we also present results analyzing the impact of the resulting changes to the synthetic stellar spectra on observable chemistry in terrestrial planet atmospheres.

==> HoudebineNotes.tex <==
Many previous studies used restricted Hydrogen atomic models

investigating changes in line profiles and formation as a function of atmospheric conditions and chromospheric structures
"the approximations typically assumed" and inability to compare to intrinsic Lya line profiles ..."incomplete understanding of the line formation and sets of constraints on the chromospheric structure"

Houdebine I
\begin{itemize}
\item investigated effects of Teff, vsini, turbulence, and temperature structure on Lya and Ha line formation in M dwarf stars
\item found a constant temperature gradient in a log(M) scale in the chromosphere and TR best reproduce observations and that a very thin TR is required to account for the observed Lya to Ha surface flux ratio (in the Sun?)
\item found that turbulence and rotational broadening have little effect on the line profiles and fluxes
\item \textbf{temperature break demarcates the temperature domains of formation of the Lyman and other Hydrogen series} and that it is the main parameter that influences the line widths and wings
\item "high resolution and high SNR observations of Ha and and estimate of the lya to Ha surface flux ratio are required to produce any meaningful model atmosphere"
\item used the NLTE radiative transfer code of Carlsson 1986 (assumes CRD)
\item relied on estimated lya to Ha surface flux ratio in lieu of Lya observations (needs to be around 1)
\end{itemize}

HoudebineII
\begin{itemize}
\item investigated the formation of hydrogen lines in high pressure stellar chromospheres
\item relied on estimated lya to Ha surface flux ratio in lieu of Lya observations, but could not match the Ha observations and the flux ratio simultaneously
\item for Hydrogen line modeling, they use observations of Ha and H beta profiles
\item found that Lya FWHM decreases with increasing pressure, and the lower pressure models show extended Lya wings
\end{itemize}

Houdebine III
\begin{itemize}
\item looked at different TR pressures and temperature minima
\item found Lya not sensitive to changes in the temperature minimum and found that the effect of the temperature break zone is only important for high pressure atmospheres 
\item found densest models produce broad profiles with no self-reversal and strong wings. When decreasing the TR pressure (below logM=-5.5), the self-reversal appears and strengthens
\end{itemize}

Houdebine V
\begin{itemize}
\item 
\end{itemize}




